A Call to Reflect on Evaluation Practices for Failure Detection in Image Classification

Reliable application of machine learning-based decision systems in the wild is one of the major challenges currently investigated by the field. A large portion of established approaches aims to detect erroneous predictions by means of assigning confidence scores. This confidence may be obtained by either quantifying the model's predictive uncertainty, learning explicit scoring functions, or assessing whether the input is in line with the training distribution. Curiously, while these approaches all state to address the same eventual goal of detecting failures of a classifier upon real-life application, they currently constitute largely separated research fields with individual evaluation protocols, which either exclude a substantial part of relevant methods or ignore large parts of relevant failure sources. In this work, we systematically reveal current pitfalls caused by these inconsistencies and derive requirements for a holistic and realistic evaluation of failure detection. To demonstrate the relevance of this unified perspective, we present a large-scale empirical study for the first time enabling benchmarking confidence scoring functions w.r.t all relevant methods and failure sources. The revelation of a simple softmax response baseline as the overall best performing method underlines the drastic shortcomings of current evaluation in the abundance of publicized research on confidence scoring. Code and trained models are at https://github.com/IML-DKFZ/fd-shifts.

==> mode_comparison.tex <==
\begin{tabular}{ll?*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}}
 & \multicolumn{1}{c}{} & \multicolumn{2}{c?}{iWildCam} & \multicolumn{6}{c?}{CIFAR-100} & \multicolumn{6}{c?}{CIFAR-10} & \multicolumn{8}{c}{SVHN} \\
 & study & \multicolumn{2}{c?}{s-ncs} & \multicolumn{2}{c?}{s-ncs} & \multicolumn{4}{c?}{ns-ncs} & \multicolumn{2}{c?}{s-ncs} & \multicolumn{4}{c?}{ns-ncs} & \multicolumn{2}{c?}{s-ncs} & \multicolumn{6}{c}{ns-ncs} \\
 & ncs-data set & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c10} & \multicolumn{2}{c?}{svhn} & \multicolumn{2}{c?}{ti} & \multicolumn{2}{c?}{c100} & \multicolumn{2}{c?}{svhn} & \multicolumn{2}{c?}{ti} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c10} & \multicolumn{2}{c?}{c100} & \multicolumn{2}{c}{ti} \\
 & ood protocol & P & O & P & O & P & O & P & O & P & O & P & O & P & O & P & O & P & O & P & O & P & O \\
\midrule
MSR & CNN & {\cellcolor[HTML]{FDD9B5}} \color[HTML]{000000} 85.5 & {\cellcolor[HTML]{FDD8B2}} \color[HTML]{000000} 77.1 & {\cellcolor[HTML]{FEE2C7}} \color[HTML]{000000} 86.4 & {\cellcolor[HTML]{FDB77A}} \color[HTML]{000000} 77.4 & {\cellcolor[HTML]{FEE2C7}} \color[HTML]{000000} 88.4 & {\cellcolor[HTML]{FDD1A4}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{E05206}} \color[HTML]{F1F1F1} 84.3 & {\cellcolor[HTML]{E15407}} \color[HTML]{F1F1F1} 74.5 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 91.7 & {\cellcolor[HTML]{D94801}} \color[HTML]{F1F1F1} 89.1 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000} 95.8 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 93.6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 96.9 & {\cellcolor[HTML]{FDAF6C}} \color[HTML]{000000} 95.2 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 93.9 & {\cellcolor[HTML]{FDCFA0}} \color[HTML]{000000} 92.2 & {\cellcolor[HTML]{963003}} \color[HTML]{F1F1F1} 97.5 & {\cellcolor[HTML]{9F3303}} \color[HTML]{F1F1F1} 96.2 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 97.3 & {\cellcolor[HTML]{9F3303}} \color[HTML]{F1F1F1} 96.0 & {\cellcolor[HTML]{963003}} \color[HTML]{F1F1F1} 97.4 & {\cellcolor[HTML]{8F2D04}} \color[HTML]{F1F1F1} 96.0 \\
MLS & CNN & {\cellcolor[HTML]{FD9B50}} \color[HTML]{000000} 82.8 & {\cellcolor[HTML]{FDD3A9}} \color[HTML]{000000} 76.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 86.8 & {\cellcolor[HTML]{FFEEDE}} \color[HTML]{000000} 78.4 & {\cellcolor[HTML]{FEDDBC}} \color[HTML]{000000} 87.9 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 79.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 93.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 87.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 92.9 & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 90.8 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 97.6 & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 96.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 98.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 97.6 & {\cellcolor[HTML]{FEE2C6}} \color[HTML]{000000} 94.3 & {\cellcolor[HTML]{FEE0C1}} \color[HTML]{000000} 92.9 & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 98.6 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 97.7 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 98.3 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 97.4 & {\cellcolor[HTML]{FEE1C4}} \color[HTML]{000000} 98.4 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 97.5 \\
PE & CNN & {\cellcolor[HTML]{FEE4CA}} \color[HTML]{000000} 86.1 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{FDC48F}} \color[HTML]{000000} 86.0 & {\cellcolor[HTML]{F67824}} \color[HTML]{F1F1F1} 76.6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1} 81.4 & {\cellcolor[HTML]{EE6410}} \color[HTML]{F1F1F1} 71.0 & {\cellcolor[HTML]{FDD7AF}} \color[HTML]{000000} 91.0 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 83.5 & {\cellcolor[HTML]{FD9A4E}} \color[HTML]{000000} 92.0 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1} 89.5 & {\cellcolor[HTML]{FDDBB8}} \color[HTML]{000000} 96.4 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 94.4 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 97.5 & {\cellcolor[HTML]{FDD3A9}} \color[HTML]{000000} 96.1 & {\cellcolor[HTML]{FDDBB8}} \color[HTML]{000000} 94.0 & {\cellcolor[HTML]{FDD1A4}} \color[HTML]{000000} 92.3 & {\cellcolor[HTML]{F26C16}} \color[HTML]{F1F1F1} 97.9 & {\cellcolor[HTML]{F06712}} \color[HTML]{F1F1F1} 96.7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 97.6 & {\cellcolor[HTML]{F06712}} \color[HTML]{F1F1F1} 96.5 & {\cellcolor[HTML]{E45709}} \color[HTML]{F1F1F1} 97.7 & {\cellcolor[HTML]{E5590A}} \color[HTML]{F1F1F1} 96.5 \\
MCD-MSR & CNN & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 85.6 & {\cellcolor[HTML]{FDCD9C}} \color[HTML]{000000} 76.4 & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 86.3 & {\cellcolor[HTML]{FDC692}} \color[HTML]{000000} 77.6 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000} 86.4 & {\cellcolor[HTML]{FDB576}} \color[HTML]{000000} 77.0 & {\cellcolor[HTML]{E75C0C}} \color[HTML]{F1F1F1} 84.8 & {\cellcolor[HTML]{EE6410}} \color[HTML]{F1F1F1} 75.7 & {\cellcolor[HTML]{F87F2C}} \color[HTML]{F1F1F1} 91.8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 89.3 & {\cellcolor[HTML]{FD9446}} \color[HTML]{000000} 94.3 & {\cellcolor[HTML]{FC8A39}} \color[HTML]{F1F1F1} 91.7 & {\cellcolor[HTML]{F9812E}} \color[HTML]{F1F1F1} 95.9 & {\cellcolor[HTML]{F77B28}} \color[HTML]{F1F1F1} 94.0 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 94.6 & {\cellcolor[HTML]{FEE5CB}} \color[HTML]{000000} 93.1 & {\cellcolor[HTML]{F26C16}} \color[HTML]{F1F1F1} 97.9 & {\cellcolor[HTML]{F06712}} \color[HTML]{F1F1F1} 96.7 & {\cellcolor[HTML]{FD9C51}} \color[HTML]{000000} 97.7 & {\cellcolor[HTML]{E5590A}} \color[HTML]{F1F1F1} 96.4 & {\cellcolor[HTML]{FD974A}} \color[HTML]{000000} 98.0 & {\cellcolor[HTML]{FB8634}} \color[HTML]{F1F1F1} 96.8 \\
MCD-MLS & CNN & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000} 84.7 & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{FDCE9E}} \color[HTML]{000000} 86.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{FEE6CE}} \color[HTML]{000000} 88.7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 80.7 & {\cellcolor[HTML]{FD9C51}} \color[HTML]{000000} 87.9 & {\cellcolor[HTML]{FDAB66}} \color[HTML]{000000} 80.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 92.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 90.9 & {\cellcolor[HTML]{FDD6AE}} \color[HTML]{000000} 96.2 & {\cellcolor[HTML]{FDD3A9}} \color[HTML]{000000} 94.3 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 98.0 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 97.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 95.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 98.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 97.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 98.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 97.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 98.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 97.8 \\
MCD-PE & CNN & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 86.8 & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{FDD5AD}} \color[HTML]{000000} 86.2 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 78.5 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 87.4 & {\cellcolor[HTML]{FDD1A4}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{FD8C3B}} \color[HTML]{F1F1F1} 87.1 & {\cellcolor[HTML]{FD9D53}} \color[HTML]{000000} 79.5 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 92.4 & {\cellcolor[HTML]{FDC590}} \color[HTML]{000000} 90.2 & {\cellcolor[HTML]{FDAE6A}} \color[HTML]{000000} 95.0 & {\cellcolor[HTML]{FDA660}} \color[HTML]{000000} 92.7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 96.9 & {\cellcolor[HTML]{FDBB81}} \color[HTML]{000000} 95.5 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 94.9 & {\cellcolor[HTML]{FEECD9}} \color[HTML]{000000} 93.5 & {\cellcolor[HTML]{FDD3A9}} \color[HTML]{000000} 98.4 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 97.5 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 98.2 & {\cellcolor[HTML]{FDCD9C}} \color[HTML]{000000} 97.2 & {\cellcolor[HTML]{FEE1C4}} \color[HTML]{000000} 98.4 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 97.5 \\
MCD-EE & CNN & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 86.8 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 78.7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 85.9 & {\cellcolor[HTML]{FEE7D1}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{FDCD9C}} \color[HTML]{000000} 86.5 & {\cellcolor[HTML]{FDC28B}} \color[HTML]{000000} 77.9 & {\cellcolor[HTML]{F87F2C}} \color[HTML]{F1F1F1} 86.5 & {\cellcolor[HTML]{FD9141}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 92.5 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 90.3 & {\cellcolor[HTML]{FDD6AE}} \color[HTML]{000000} 96.2 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 94.4 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 97.5 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 96.3 & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 95.1 & {\cellcolor[HTML]{FFEFDF}} \color[HTML]{000000} 93.7 & {\cellcolor[HTML]{FEE1C4}} \color[HTML]{000000} 98.5 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 97.6 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 98.2 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 97.3 & {\cellcolor[HTML]{FEE1C4}} \color[HTML]{000000} 98.4 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 97.5 \\
MCD-MI & CNN & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 76.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 67.8 & {\cellcolor[HTML]{FD9C51}} \color[HTML]{000000} 85.6 & {\cellcolor[HTML]{FEDEBF}} \color[HTML]{000000} 78.0 & {\cellcolor[HTML]{FEE5CC}} \color[HTML]{000000} 88.6 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 81.6 & {\cellcolor[HTML]{FD9A4E}} \color[HTML]{000000} 87.8 & {\cellcolor[HTML]{FDB87C}} \color[HTML]{000000} 81.4 & {\cellcolor[HTML]{EC620F}} \color[HTML]{F1F1F1} 91.6 & {\cellcolor[HTML]{E15307}} \color[HTML]{F1F1F1} 89.2 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 90.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 87.1 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 93.7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 91.2 & {\cellcolor[HTML]{FEE2C6}} \color[HTML]{000000} 94.3 & {\cellcolor[HTML]{FEDEBD}} \color[HTML]{000000} 92.8 & {\cellcolor[HTML]{E45709}} \color[HTML]{F1F1F1} 97.8 & {\cellcolor[HTML]{E5590A}} \color[HTML]{F1F1F1} 96.6 & {\cellcolor[HTML]{F87D29}} \color[HTML]{F1F1F1} 97.5 & {\cellcolor[HTML]{DB4B03}} \color[HTML]{F1F1F1} 96.3 & {\cellcolor[HTML]{FDAC67}} \color[HTML]{000000} 98.1 & {\cellcolor[HTML]{FDB06E}} \color[HTML]{000000} 97.1 \\
ConfidNet & CNN & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 86.6 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 78.5 & {\cellcolor[HTML]{FDCE9E}} \color[HTML]{000000} 86.1 & {\cellcolor[HTML]{DA4902}} \color[HTML]{F1F1F1} 76.0 & {\cellcolor[HTML]{FDCD9C}} \color[HTML]{000000} 86.5 & {\cellcolor[HTML]{FDA55F}} \color[HTML]{000000} 75.8 & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 91.4 & {\cellcolor[HTML]{FDD2A6}} \color[HTML]{000000} 83.2 & {\cellcolor[HTML]{FDB576}} \color[HTML]{000000} 92.2 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1} 89.5 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 96.3 & {\cellcolor[HTML]{FDCB9B}} \color[HTML]{000000} 94.0 & {\cellcolor[HTML]{FDC590}} \color[HTML]{000000} 97.1 & {\cellcolor[HTML]{FDB77A}} \color[HTML]{000000} 95.4 & {\cellcolor[HTML]{FDDBB8}} \color[HTML]{000000} 94.0 & {\cellcolor[HTML]{FDD4AA}} \color[HTML]{000000} 92.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 96.0 & {\cellcolor[HTML]{DE5005}} \color[HTML]{F1F1F1} 97.2 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 95.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 95.9 \\
DG-MCD-MSR & CNN & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 87.6 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 78.5 & {\cellcolor[HTML]{FDD5AD}} \color[HTML]{000000} 86.2 & {\cellcolor[HTML]{FDAF6C}} \color[HTML]{000000} 77.3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000} 86.7 & {\cellcolor[HTML]{FDBA7F}} \color[HTML]{000000} 77.4 & {\cellcolor[HTML]{D34601}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{DF5106}} \color[HTML]{F1F1F1} 74.3 & {\cellcolor[HTML]{B03903}} \color[HTML]{F1F1F1} 91.2 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 88.5 & {\cellcolor[HTML]{F4711C}} \color[HTML]{F1F1F1} 93.4 & {\cellcolor[HTML]{F26C16}} \color[HTML]{F1F1F1} 90.7 & {\cellcolor[HTML]{D04501}} \color[HTML]{F1F1F1} 94.8 & {\cellcolor[HTML]{D34601}} \color[HTML]{F1F1F1} 92.7 & {\cellcolor[HTML]{FEEAD5}} \color[HTML]{000000} 94.7 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 93.2 & {\cellcolor[HTML]{E45709}} \color[HTML]{F1F1F1} 97.8 & {\cellcolor[HTML]{E5590A}} \color[HTML]{F1F1F1} 96.6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 97.6 & {\cellcolor[HTML]{DB4B03}} \color[HTML]{F1F1F1} 96.3 & {\cellcolor[HTML]{F26C16}} \color[HTML]{F1F1F1} 97.8 & {\cellcolor[HTML]{F06712}} \color[HTML]{F1F1F1} 96.6 \\
DG-Res & CNN & {\cellcolor[HTML]{FDD8B2}} \color[HTML]{000000} 85.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 79.5 & {\cellcolor[HTML]{A13403}} \color[HTML]{F1F1F1} 84.4 & {\cellcolor[HTML]{FC8937}} \color[HTML]{F1F1F1} 76.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 90.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 84.1 & {\cellcolor[HTML]{FDB373}} \color[HTML]{000000} 89.1 & {\cellcolor[HTML]{FDC692}} \color[HTML]{000000} 82.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 90.9 & {\cellcolor[HTML]{A63603}} \color[HTML]{F1F1F1} 88.8 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 97.6 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 96.3 & {\cellcolor[HTML]{FEE2C7}} \color[HTML]{000000} 97.8 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 96.9 & {\cellcolor[HTML]{FEE0C1}} \color[HTML]{000000} 94.2 & {\cellcolor[HTML]{FEDEBD}} \color[HTML]{000000} 92.8 & {\cellcolor[HTML]{FEE1C4}} \color[HTML]{000000} 98.5 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 97.7 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 98.3 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 97.5 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 98.2 & {\cellcolor[HTML]{FDCD9C}} \color[HTML]{000000} 97.3 \\
Devries et al. & CNN & {\cellcolor[HTML]{F26C16}} \color[HTML]{F1F1F1} 81.0 & {\cellcolor[HTML]{FD8F3E}} \color[HTML]{F1F1F1} 73.7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 84.1 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 75.1 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 74.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 63.7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 80.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 69.0 & {\cellcolor[HTML]{F87F2C}} \color[HTML]{F1F1F1} 91.8 & {\cellcolor[HTML]{E15307}} \color[HTML]{F1F1F1} 89.2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 97.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 96.5 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 97.5 & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 96.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 88.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.4 & {\cellcolor[HTML]{F06712}} \color[HTML]{F1F1F1} 96.7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 96.7 & {\cellcolor[HTML]{8F2D04}} \color[HTML]{F1F1F1} 95.9 & {\cellcolor[HTML]{B13A03}} \color[HTML]{F1F1F1} 97.5 & {\cellcolor[HTML]{FB8634}} \color[HTML]{F1F1F1} 96.8 \\
\midrule \\
MSR & ViT & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 86.1 & {\cellcolor[HTML]{FDAD69}} \color[HTML]{000000} 74.2 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 91.9 & {\cellcolor[HTML]{F36E19}} \color[HTML]{F1F1F1} 89.0 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 93.8 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000} 91.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 89.7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 86.5 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 97.2 & {\cellcolor[HTML]{FDA159}} \color[HTML]{000000} 96.7 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 98.8 & {\cellcolor[HTML]{FDBD83}} \color[HTML]{000000} 98.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 95.3 & {\cellcolor[HTML]{902E04}} \color[HTML]{F1F1F1} 94.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 93.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 93.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 98.1 & {\cellcolor[HTML]{8F2D04}} \color[HTML]{F1F1F1} 97.4 & {\cellcolor[HTML]{963003}} \color[HTML]{F1F1F1} 98.0 & {\cellcolor[HTML]{9E3303}} \color[HTML]{F1F1F1} 97.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 98.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.7 \\
MLS & ViT & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 86.5 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 76.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.3 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 92.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 95.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 93.7 & {\cellcolor[HTML]{E05206}} \color[HTML]{F1F1F1} 91.2 & {\cellcolor[HTML]{F26C16}} \color[HTML]{F1F1F1} 89.2 & {\cellcolor[HTML]{FDC895}} \color[HTML]{000000} 97.5 & {\cellcolor[HTML]{FDD1A4}} \color[HTML]{000000} 97.3 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 99.5 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 99.4 & {\cellcolor[HTML]{D14501}} \color[HTML]{F1F1F1} 96.0 & {\cellcolor[HTML]{E45709}} \color[HTML]{F1F1F1} 95.7 & {\cellcolor[HTML]{A23503}} \color[HTML]{F1F1F1} 94.2 & {\cellcolor[HTML]{B53B02}} \color[HTML]{F1F1F1} 93.6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 98.7 & {\cellcolor[HTML]{FD9446}} \color[HTML]{000000} 98.3 & {\cellcolor[HTML]{F98230}} \color[HTML]{F1F1F1} 98.5 & {\cellcolor[HTML]{FD9A4E}} \color[HTML]{000000} 98.2 & {\cellcolor[HTML]{FEE3C8}} \color[HTML]{000000} 99.0 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 98.7 \\
PE & ViT & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 86.6 & {\cellcolor[HTML]{FDC48F}} \color[HTML]{000000} 75.1 & {\cellcolor[HTML]{FB8634}} \color[HTML]{F1F1F1} 92.2 & {\cellcolor[HTML]{FA8532}} \color[HTML]{F1F1F1} 89.5 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 94.2 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 91.6 & {\cellcolor[HTML]{902E04}} \color[HTML]{F1F1F1} 90.0 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 87.0 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 97.2 & {\cellcolor[HTML]{FDA159}} \color[HTML]{000000} 96.7 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 98.8 & {\cellcolor[HTML]{FDBD83}} \color[HTML]{000000} 98.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 95.3 & {\cellcolor[HTML]{902E04}} \color[HTML]{F1F1F1} 94.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 93.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 93.0 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1} 98.2 & {\cellcolor[HTML]{8F2D04}} \color[HTML]{F1F1F1} 97.4 & {\cellcolor[HTML]{B13A03}} \color[HTML]{F1F1F1} 98.1 & {\cellcolor[HTML]{9E3303}} \color[HTML]{F1F1F1} 97.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 98.4 & {\cellcolor[HTML]{9B3203}} \color[HTML]{F1F1F1} 97.8 \\
MCD-MSR & ViT & {\cellcolor[HTML]{FEE4CA}} \color[HTML]{000000} 84.5 & {\cellcolor[HTML]{FDCFA0}} \color[HTML]{000000} 75.5 & {\cellcolor[HTML]{CE4401}} \color[HTML]{F1F1F1} 91.2 & {\cellcolor[HTML]{CD4401}} \color[HTML]{F1F1F1} 87.9 & {\cellcolor[HTML]{B33B02}} \color[HTML]{F1F1F1} 89.0 & {\cellcolor[HTML]{B03903}} \color[HTML]{F1F1F1} 85.2 & {\cellcolor[HTML]{FDA159}} \color[HTML]{000000} 92.7 & {\cellcolor[HTML]{F87D29}} \color[HTML]{F1F1F1} 89.6 & {\cellcolor[HTML]{B33B02}} \color[HTML]{F1F1F1} 96.1 & {\cellcolor[HTML]{B03903}} \color[HTML]{F1F1F1} 95.3 & {\cellcolor[HTML]{D14501}} \color[HTML]{F1F1F1} 97.6 & {\cellcolor[HTML]{C64102}} \color[HTML]{F1F1F1} 96.8 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1} 95.8 & {\cellcolor[HTML]{AB3803}} \color[HTML]{F1F1F1} 95.1 & {\cellcolor[HTML]{FC8937}} \color[HTML]{F1F1F1} 95.5 & {\cellcolor[HTML]{F9812E}} \color[HTML]{F1F1F1} 94.7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 98.1 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.3 & {\cellcolor[HTML]{963003}} \color[HTML]{F1F1F1} 98.0 & {\cellcolor[HTML]{9E3303}} \color[HTML]{F1F1F1} 97.3 & {\cellcolor[HTML]{AD3803}} \color[HTML]{F1F1F1} 98.5 & {\cellcolor[HTML]{9B3203}} \color[HTML]{F1F1F1} 97.8 \\
MCD-MLS & ViT & {\cellcolor[HTML]{FEE3C8}} \color[HTML]{000000} 84.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 78.1 & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 94.0 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 92.1 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 93.7 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 91.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.9 & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 93.2 & {\cellcolor[HTML]{FDD2A6}} \color[HTML]{000000} 97.6 & {\cellcolor[HTML]{FDD1A4}} \color[HTML]{000000} 97.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 99.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 99.5 & {\cellcolor[HTML]{FDD3A9}} \color[HTML]{000000} 97.6 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 97.3 & {\cellcolor[HTML]{FDAF6C}} \color[HTML]{000000} 96.0 & {\cellcolor[HTML]{FDBB81}} \color[HTML]{000000} 95.5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 98.9 & {\cellcolor[HTML]{FDB06E}} \color[HTML]{000000} 98.5 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 98.8 & {\cellcolor[HTML]{FDB576}} \color[HTML]{000000} 98.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 99.1 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 98.7 \\
MCD-PE & ViT & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 85.3 & {\cellcolor[HTML]{FEE6CE}} \color[HTML]{000000} 76.8 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 91.9 & {\cellcolor[HTML]{F36E19}} \color[HTML]{F1F1F1} 89.0 & {\cellcolor[HTML]{DE4E05}} \color[HTML]{F1F1F1} 89.9 & {\cellcolor[HTML]{E15307}} \color[HTML]{F1F1F1} 86.6 & {\cellcolor[HTML]{FDC692}} \color[HTML]{000000} 93.4 & {\cellcolor[HTML]{FDAF6C}} \color[HTML]{000000} 90.9 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 96.2 & {\cellcolor[HTML]{C94202}} \color[HTML]{F1F1F1} 95.5 & {\cellcolor[HTML]{DC4C03}} \color[HTML]{F1F1F1} 97.7 & {\cellcolor[HTML]{DB4B03}} \color[HTML]{F1F1F1} 97.0 & {\cellcolor[HTML]{D14501}} \color[HTML]{F1F1F1} 96.0 & {\cellcolor[HTML]{C14002}} \color[HTML]{F1F1F1} 95.3 & {\cellcolor[HTML]{FD9141}} \color[HTML]{000000} 95.6 & {\cellcolor[HTML]{FC8937}} \color[HTML]{F1F1F1} 94.8 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1} 98.3 & {\cellcolor[HTML]{B33B02}} \color[HTML]{F1F1F1} 97.6 & {\cellcolor[HTML]{D14501}} \color[HTML]{F1F1F1} 98.2 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 97.5 & {\cellcolor[HTML]{E05206}} \color[HTML]{F1F1F1} 98.6 & {\cellcolor[HTML]{DD4D04}} \color[HTML]{F1F1F1} 98.0 \\
MCD-EE & ViT & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 85.3 & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 77.1 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 92.3 & {\cellcolor[HTML]{FC8937}} \color[HTML]{F1F1F1} 89.6 & {\cellcolor[HTML]{ED6310}} \color[HTML]{F1F1F1} 90.5 & {\cellcolor[HTML]{F26B15}} \color[HTML]{F1F1F1} 87.5 & {\cellcolor[HTML]{FDD3A9}} \color[HTML]{000000} 93.7 & {\cellcolor[HTML]{FDC38D}} \color[HTML]{000000} 91.4 & {\cellcolor[HTML]{E65A0B}} \color[HTML]{F1F1F1} 96.5 & {\cellcolor[HTML]{EF6612}} \color[HTML]{F1F1F1} 96.0 & {\cellcolor[HTML]{F98230}} \color[HTML]{F1F1F1} 98.2 & {\cellcolor[HTML]{F77B28}} \color[HTML]{F1F1F1} 97.6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 96.3 & {\cellcolor[HTML]{E45709}} \color[HTML]{F1F1F1} 95.7 & {\cellcolor[HTML]{FDA057}} \color[HTML]{000000} 95.8 & {\cellcolor[HTML]{FD984B}} \color[HTML]{000000} 95.0 & {\cellcolor[HTML]{D94801}} \color[HTML]{F1F1F1} 98.4 & {\cellcolor[HTML]{DB4B03}} \color[HTML]{F1F1F1} 97.8 & {\cellcolor[HTML]{F26C16}} \color[HTML]{F1F1F1} 98.4 & {\cellcolor[HTML]{EC620F}} \color[HTML]{F1F1F1} 97.8 & {\cellcolor[HTML]{FDA057}} \color[HTML]{000000} 98.8 & {\cellcolor[HTML]{F9802D}} \color[HTML]{F1F1F1} 98.2 \\
MCD-MI & ViT & {\cellcolor[HTML]{FEE7D0}} \color[HTML]{000000} 84.8 & {\cellcolor[HTML]{FDC997}} \color[HTML]{000000} 75.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 90.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 86.5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 87.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 83.7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 92.3 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 89.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 95.7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 94.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 96.1 & {\cellcolor[HTML]{892B04}} \color[HTML]{F1F1F1} 95.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 94.6 & {\cellcolor[HTML]{FC8937}} \color[HTML]{F1F1F1} 95.5 & {\cellcolor[HTML]{F67925}} \color[HTML]{F1F1F1} 94.6 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 98.1 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.1 & {\cellcolor[HTML]{AD3803}} \color[HTML]{F1F1F1} 98.5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 97.7 \\
MAHA & ViT & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 71.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 67.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 92.9 & {\cellcolor[HTML]{E15307}} \color[HTML]{F1F1F1} 90.0 & {\cellcolor[HTML]{F26D17}} \color[HTML]{F1F1F1} 87.6 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 94.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 93.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 98.2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 98.1 & {\cellcolor[HTML]{D14501}} \color[HTML]{F1F1F1} 97.6 & {\cellcolor[HTML]{F26B15}} \color[HTML]{F1F1F1} 97.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 98.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 98.2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 97.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 96.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 99.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 99.2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 99.2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 99.1 & {\cellcolor[HTML]{FDC692}} \color[HTML]{000000} 98.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 98.8 \\
\bottomrule
\end{tabular}

==> paper_results_fail-NLL.tex <==
\begin{tabular}{ll?rrr?xx?xx?rrrrrr?rrrrr?rrrrr}
 & \multicolumn{1}{c}{} & \multicolumn{3}{c}{iWildCam} & \multicolumn{2}{c}{BREEDS} & \multicolumn{2}{c}{CAMELYON} & \multicolumn{6}{c}{CIFAR-100} & \multicolumn{5}{c}{CIFAR-10} & \multicolumn{5}{c}{SVHN} \\
 & study & iid & sub & s-ncs & iid & sub & iid & sub & iid & sub & cor & s-ncs & \multicolumn{2}{c?}{ns-ncs} & iid & cor & s-ncs & \multicolumn{2}{c?}{ns-ncs} & iid & s-ncs & \multicolumn{3}{c}{ns-ncs} \\
 & ncs-data set &  &  &  &  &  &  &  &  &  &  & c10 & svhn & ti &  &  & c100 & svhn & ti &  &  & c10 & c100 & ti \\
\midrule
MSR & CNN & {\cellcolor[HTML]{FEE7D1}} \color[HTML]{000000} 0.54 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 0.45 & {\cellcolor[HTML]{FDD3A7}} \color[HTML]{000000} 0.74 & {\cellcolor[HTML]{FDAF6C}} \color[HTML]{000000} 0.18 & {\cellcolor[HTML]{B83C02}} \color[HTML]{F1F1F1} 0.92 & {\cellcolor[HTML]{FDD2A6}} \color[HTML]{000000} 0.16 & {\cellcolor[HTML]{FEE0C1}} \color[HTML]{000000} 0.65 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 0.41 & {\cellcolor[HTML]{FDD8B2}} \color[HTML]{000000} 1.05 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{FEEDDB}} \color[HTML]{000000} 0.83 & {\cellcolor[HTML]{FEEDDB}} \color[HTML]{000000} 0.91 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 0.94 & {\cellcolor[HTML]{FDC38D}} \color[HTML]{000000} 0.15 & {\cellcolor[HTML]{F9812E}} \color[HTML]{F1F1F1} 0.58 & {\cellcolor[HTML]{D94801}} \color[HTML]{F1F1F1} 1.53 & {\cellcolor[HTML]{C14002}} \color[HTML]{F1F1F1} 1.44 & {\cellcolor[HTML]{AB3803}} \color[HTML]{F1F1F1} 0.84 & {\cellcolor[HTML]{FEE5CC}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FDA55F}} \color[HTML]{000000} 1.41 & {\cellcolor[HTML]{FEDEBD}} \color[HTML]{000000} 0.50 & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 0.53 & {\cellcolor[HTML]{FEDDBC}} \color[HTML]{000000} 0.52 \\
MLS & CNN & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 0.44 & {\cellcolor[HTML]{FEECD9}} \color[HTML]{000000} 0.44 & {\cellcolor[HTML]{FFEEDE}} \color[HTML]{000000} 0.51 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 0.17 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.64 & {\cellcolor[HTML]{FDD2A6}} \color[HTML]{000000} 0.16 & {\cellcolor[HTML]{FDD7AF}} \color[HTML]{000000} 0.68 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 0.41 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.56 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.54 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.58 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.64 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.40 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 0.14 & {\cellcolor[HTML]{FFEEDE}} \color[HTML]{000000} 0.41 & {\cellcolor[HTML]{FDCD9C}} \color[HTML]{000000} 0.83 & {\cellcolor[HTML]{FDB77A}} \color[HTML]{000000} 0.72 & {\cellcolor[HTML]{FDCE9E}} \color[HTML]{000000} 0.40 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.11 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.29 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.26 & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 0.28 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.28 \\
PE & CNN & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.42 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.40 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 0.47 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 0.17 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{FDD2A6}} \color[HTML]{000000} 0.16 & {\cellcolor[HTML]{FDD1A4}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{FFEFE0}} \color[HTML]{000000} 0.43 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.60 & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 0.62 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 0.67 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 0.96 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.50 & {\cellcolor[HTML]{FDC38D}} \color[HTML]{000000} 0.15 & {\cellcolor[HTML]{FDC692}} \color[HTML]{000000} 0.49 & {\cellcolor[HTML]{FD9E54}} \color[HTML]{000000} 1.08 & {\cellcolor[HTML]{F9812E}} \color[HTML]{F1F1F1} 1.03 & {\cellcolor[HTML]{FDA45D}} \color[HTML]{000000} 0.51 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.11 & {\cellcolor[HTML]{FFEEDE}} \color[HTML]{000000} 0.43 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 0.37 & {\cellcolor[HTML]{FEECD9}} \color[HTML]{000000} 0.38 & {\cellcolor[HTML]{FEEBD7}} \color[HTML]{000000} 0.38 \\
MCD-MSR & CNN & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 0.40 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.35 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 0.58 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 0.16 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 0.79 & {\cellcolor[HTML]{FEE7D0}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FEDCBB}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.37 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.52 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.58 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 0.62 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.12 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.39 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 0.89 & {\cellcolor[HTML]{FB8735}} \color[HTML]{F1F1F1} 1.00 & {\cellcolor[HTML]{FA8331}} \color[HTML]{F1F1F1} 0.60 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.10 & {\cellcolor[HTML]{FDD1A4}} \color[HTML]{000000} 0.95 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.29 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 0.30 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.28 \\
MCD-MLS & CNN & {\cellcolor[HTML]{FFEFE0}} \color[HTML]{000000} 0.45 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 0.45 & {\cellcolor[HTML]{FFF3E7}} \color[HTML]{000000} 0.46 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 0.17 & {\cellcolor[HTML]{FFEEDE}} \color[HTML]{000000} 0.65 & {\cellcolor[HTML]{FEE7D0}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FDC48F}} \color[HTML]{000000} 0.73 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 0.41 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.60 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.62 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.40 & {\cellcolor[HTML]{FDCD9C}} \color[HTML]{000000} 0.83 & {\cellcolor[HTML]{FD9243}} \color[HTML]{000000} 0.94 & {\cellcolor[HTML]{FDB77A}} \color[HTML]{000000} 0.46 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.11 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.27 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.25 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.26 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.25 \\
MCD-PE & CNN & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.39 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 0.39 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.44 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 0.17 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{FEE7D0}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FDC48F}} \color[HTML]{000000} 0.73 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 0.41 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.56 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.60 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{FFEEDE}} \color[HTML]{000000} 0.58 & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 0.42 & {\cellcolor[HTML]{FDC088}} \color[HTML]{000000} 0.90 & {\cellcolor[HTML]{F67824}} \color[HTML]{F1F1F1} 1.08 & {\cellcolor[HTML]{FDA45D}} \color[HTML]{000000} 0.51 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.10 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.35 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.25 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.27 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.25 \\
MCD-EE & CNN & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 0.40 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.40 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.44 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 0.17 & {\cellcolor[HTML]{FDD4AA}} \color[HTML]{000000} 0.71 & {\cellcolor[HTML]{FEE7D0}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FDC48F}} \color[HTML]{000000} 0.73 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 0.41 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 0.57 & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 0.56 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 0.62 & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 0.75 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 0.61 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 0.14 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 0.42 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 0.89 & {\cellcolor[HTML]{FD9F56}} \color[HTML]{000000} 0.86 & {\cellcolor[HTML]{FDC692}} \color[HTML]{000000} 0.42 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.11 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.35 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.25 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.27 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.26 \\
MCD-MI & CNN & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.38 & {\cellcolor[HTML]{FFEFDF}} \color[HTML]{000000} 0.41 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 0.58 & {\cellcolor[HTML]{FDAF6C}} \color[HTML]{000000} 0.18 & {\cellcolor[HTML]{FDBF86}} \color[HTML]{000000} 0.74 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 0.15 & {\cellcolor[HTML]{FD9C51}} \color[HTML]{000000} 0.82 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.42 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 0.57 & {\cellcolor[HTML]{FFF3E7}} \color[HTML]{000000} 0.57 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 0.61 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 0.14 & {\cellcolor[HTML]{FDC692}} \color[HTML]{000000} 0.49 & {\cellcolor[HTML]{FDAF6C}} \color[HTML]{000000} 0.99 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.74 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.94 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.10 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 0.37 & {\cellcolor[HTML]{FFEFE0}} \color[HTML]{000000} 0.32 & {\cellcolor[HTML]{FFEFE0}} \color[HTML]{000000} 0.33 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.28 \\
ConfidNet & CNN & {\cellcolor[HTML]{F57622}} \color[HTML]{F1F1F1} 1.19 & {\cellcolor[HTML]{EB600E}} \color[HTML]{F1F1F1} 1.08 & {\cellcolor[HTML]{FDD5AD}} \color[HTML]{000000} 0.72 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 0.17 & {\cellcolor[HTML]{E05206}} \color[HTML]{F1F1F1} 0.88 & {\cellcolor[HTML]{FEE7D0}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.39 & {\cellcolor[HTML]{FEE4CA}} \color[HTML]{000000} 0.89 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.60 & {\cellcolor[HTML]{FEEDDB}} \color[HTML]{000000} 0.83 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 1.00 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.54 & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FDD4AA}} \color[HTML]{000000} 0.47 & {\cellcolor[HTML]{FA8331}} \color[HTML]{F1F1F1} 1.22 & {\cellcolor[HTML]{F87F2C}} \color[HTML]{F1F1F1} 1.04 & {\cellcolor[HTML]{F77B28}} \color[HTML]{F1F1F1} 0.62 & {\cellcolor[HTML]{FEE5CC}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{FD9243}} \color[HTML]{000000} 1.62 & {\cellcolor[HTML]{FEDDBC}} \color[HTML]{000000} 0.51 & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 0.53 & {\cellcolor[HTML]{FEDDBC}} \color[HTML]{000000} 0.52 \\
DG-MCD-MSR & CNN & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 0.43 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 0.39 & {\cellcolor[HTML]{FDC38D}} \color[HTML]{000000} 0.82 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.15 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 0.79 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.10 & {\cellcolor[HTML]{F9812E}} \color[HTML]{F1F1F1} 0.88 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.36 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.53 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 0.61 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{FEEBD7}} \color[HTML]{000000} 0.69 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.12 & {\cellcolor[HTML]{FEE7D1}} \color[HTML]{000000} 0.43 & {\cellcolor[HTML]{FDA863}} \color[HTML]{000000} 1.02 & {\cellcolor[HTML]{ED6310}} \color[HTML]{F1F1F1} 1.19 & {\cellcolor[HTML]{E05206}} \color[HTML]{F1F1F1} 0.73 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.10 & {\cellcolor[HTML]{FDDAB6}} \color[HTML]{000000} 0.81 & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 0.30 & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 0.31 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 0.29 \\
DG-Res & CNN & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.78 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.46 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.71 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.23 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.98 & {\cellcolor[HTML]{FEE7D0}} \color[HTML]{000000} 0.13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.16 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.75 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 3.01 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 3.43 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 4.02 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 4.70 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 3.64 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 0.17 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.74 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.89 & {\cellcolor[HTML]{A13403}} \color[HTML]{F1F1F1} 1.57 & {\cellcolor[HTML]{B03903}} \color[HTML]{F1F1F1} 0.83 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.33 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 3.07 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.70 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.73 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.76 \\
Devries et al. & CNN & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 0.51 & {\cellcolor[HTML]{FEE7D1}} \color[HTML]{000000} 0.48 & {\cellcolor[HTML]{FEDEBD}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 0.19 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.35 & {\cellcolor[HTML]{FEE2C7}} \color[HTML]{000000} 0.64 & {\cellcolor[HTML]{FEEDDB}} \color[HTML]{000000} 0.46 & {\cellcolor[HTML]{FFEFE0}} \color[HTML]{000000} 0.67 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 0.77 & {\cellcolor[HTML]{FEEDDB}} \color[HTML]{000000} 0.83 & {\cellcolor[HTML]{FDDAB6}} \color[HTML]{000000} 1.41 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 0.91 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.22 & {\cellcolor[HTML]{FDBF86}} \color[HTML]{000000} 0.50 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.45 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.19 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.21 & {\cellcolor[HTML]{B93D02}} \color[HTML]{F1F1F1} 0.29 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 0.46 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.25 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.26 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.25 \\
\midrule \\
MSR & ViT & {\cellcolor[HTML]{E05206}} \color[HTML]{F1F1F1} 0.78 & {\cellcolor[HTML]{EB610F}} \color[HTML]{F1F1F1} 0.63 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.64 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.15 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.72 & {\cellcolor[HTML]{812804}} \color[HTML]{F1F1F1} 0.02 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 1.19 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.39 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.87 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.87 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 2.13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 2.54 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 2.46 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.10 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.52 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 3.62 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 4.52 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 3.89 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.17 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 3.21 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.23 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.23 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 1.11 \\
MLS & ViT & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.47 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.43 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.49 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.07 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 0.64 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.01 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.22 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.43 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.39 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.68 & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 0.68 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.04 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.17 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.72 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.61 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.80 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.28 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.25 & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 0.26 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.21 \\
PE & ViT & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.46 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.42 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 0.56 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 0.81 & {\cellcolor[HTML]{812804}} \color[HTML]{F1F1F1} 0.02 & {\cellcolor[HTML]{FEEDDB}} \color[HTML]{000000} 0.75 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 0.23 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.43 & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 0.48 & {\cellcolor[HTML]{FDD9B5}} \color[HTML]{000000} 0.86 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 1.07 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 0.96 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 0.06 & {\cellcolor[HTML]{FDBF86}} \color[HTML]{000000} 0.28 & {\cellcolor[HTML]{FDAD69}} \color[HTML]{000000} 1.83 & {\cellcolor[HTML]{FA8331}} \color[HTML]{F1F1F1} 2.69 & {\cellcolor[HTML]{FDAB66}} \color[HTML]{000000} 1.91 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 0.09 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 0.52 & {\cellcolor[HTML]{FD9E54}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{FD9E54}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{FD9C51}} \color[HTML]{000000} 0.61 \\
MCD-MSR & ViT & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.91 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 0.74 & {\cellcolor[HTML]{F4721E}} \color[HTML]{F1F1F1} 1.17 & {\cellcolor[HTML]{FDAF6C}} \color[HTML]{000000} 0.10 & {\cellcolor[HTML]{FDA057}} \color[HTML]{000000} 1.06 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.01 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 3.38 & {\cellcolor[HTML]{FDD3A7}} \color[HTML]{000000} 0.26 & {\cellcolor[HTML]{FDB170}} \color[HTML]{000000} 0.59 & {\cellcolor[HTML]{FDA863}} \color[HTML]{000000} 0.58 & {\cellcolor[HTML]{FC8937}} \color[HTML]{F1F1F1} 1.36 & {\cellcolor[HTML]{AE3903}} \color[HTML]{F1F1F1} 2.27 & {\cellcolor[HTML]{FDBA7F}} \color[HTML]{000000} 1.17 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 0.07 & {\cellcolor[HTML]{FC8937}} \color[HTML]{F1F1F1} 0.35 & {\cellcolor[HTML]{FA8532}} \color[HTML]{F1F1F1} 2.26 & {\cellcolor[HTML]{FD8F3E}} \color[HTML]{F1F1F1} 2.54 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 2.27 & {\cellcolor[HTML]{F87D29}} \color[HTML]{F1F1F1} 0.13 & {\cellcolor[HTML]{F26B15}} \color[HTML]{F1F1F1} 2.07 & {\cellcolor[HTML]{FC8B3A}} \color[HTML]{F1F1F1} 0.73 & {\cellcolor[HTML]{FC8937}} \color[HTML]{F1F1F1} 0.74 & {\cellcolor[HTML]{FD9649}} \color[HTML]{000000} 0.63 \\
MCD-MLS & ViT & {\cellcolor[HTML]{FEE5CB}} \color[HTML]{000000} 0.52 & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 0.48 & {\cellcolor[HTML]{FFF3E7}} \color[HTML]{000000} 0.51 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.57 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.01 & {\cellcolor[HTML]{F06712}} \color[HTML]{F1F1F1} 2.33 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 0.23 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.44 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 0.43 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 0.59 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 0.81 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.53 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 0.05 & {\cellcolor[HTML]{FEE7D1}} \color[HTML]{000000} 0.21 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.78 & {\cellcolor[HTML]{FFF3E7}} \color[HTML]{000000} 0.68 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.76 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.23 & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 0.26 & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 0.26 & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 0.24 \\
MCD-PE & ViT & {\cellcolor[HTML]{FEEBD7}} \color[HTML]{000000} 0.50 & {\cellcolor[HTML]{FDD6AE}} \color[HTML]{000000} 0.49 & {\cellcolor[HTML]{FFEFDF}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 0.71 & {\cellcolor[HTML]{812804}} \color[HTML]{F1F1F1} 0.02 & {\cellcolor[HTML]{F67723}} \color[HTML]{F1F1F1} 2.18 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.22 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.44 & {\cellcolor[HTML]{FEE2C7}} \color[HTML]{000000} 0.46 & {\cellcolor[HTML]{FEE4CA}} \color[HTML]{000000} 0.77 & {\cellcolor[HTML]{FDC895}} \color[HTML]{000000} 1.20 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 0.05 & {\cellcolor[HTML]{FDB77A}} \color[HTML]{000000} 0.29 & {\cellcolor[HTML]{FDCE9E}} \color[HTML]{000000} 1.47 & {\cellcolor[HTML]{FDAB66}} \color[HTML]{000000} 2.13 & {\cellcolor[HTML]{FDCE9E}} \color[HTML]{000000} 1.50 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 0.44 & {\cellcolor[HTML]{FDD3A7}} \color[HTML]{000000} 0.46 & {\cellcolor[HTML]{FDD3A7}} \color[HTML]{000000} 0.46 & {\cellcolor[HTML]{FDD7AF}} \color[HTML]{000000} 0.40 \\
MCD-EE & ViT & {\cellcolor[HTML]{FEE5CB}} \color[HTML]{000000} 0.52 & {\cellcolor[HTML]{FDC895}} \color[HTML]{000000} 0.51 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 0.56 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 0.76 & {\cellcolor[HTML]{812804}} \color[HTML]{F1F1F1} 0.02 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1} 2.20 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 0.23 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 0.45 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 0.47 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 0.72 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 1.10 & {\cellcolor[HTML]{FFEFDF}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 0.06 & {\cellcolor[HTML]{FDAF6C}} \color[HTML]{000000} 0.30 & {\cellcolor[HTML]{FDDAB6}} \color[HTML]{000000} 1.28 & {\cellcolor[HTML]{FDC794}} \color[HTML]{000000} 1.71 & {\cellcolor[HTML]{FDD9B5}} \color[HTML]{000000} 1.30 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 0.42 & {\cellcolor[HTML]{FDD9B5}} \color[HTML]{000000} 0.42 & {\cellcolor[HTML]{FDD9B5}} \color[HTML]{000000} 0.42 & {\cellcolor[HTML]{FDDBB8}} \color[HTML]{000000} 0.38 \\
MCD-MI & ViT & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 0.51 & {\cellcolor[HTML]{FDD6AE}} \color[HTML]{000000} 0.49 & {\cellcolor[HTML]{FEECD9}} \color[HTML]{000000} 0.58 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FEE2C7}} \color[HTML]{000000} 0.74 & {\cellcolor[HTML]{812804}} \color[HTML]{F1F1F1} 0.02 & {\cellcolor[HTML]{F87D29}} \color[HTML]{F1F1F1} 2.13 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 0.23 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 0.44 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 0.49 & {\cellcolor[HTML]{FDC895}} \color[HTML]{000000} 0.99 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 1.53 & {\cellcolor[HTML]{FEE2C7}} \color[HTML]{000000} 0.81 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 0.05 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 0.31 & {\cellcolor[HTML]{FDAC67}} \color[HTML]{000000} 1.84 & {\cellcolor[HTML]{F87F2C}} \color[HTML]{F1F1F1} 2.75 & {\cellcolor[HTML]{FDB06E}} \color[HTML]{000000} 1.85 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 0.46 & {\cellcolor[HTML]{FDBE84}} \color[HTML]{000000} 0.54 & {\cellcolor[HTML]{FDB678}} \color[HTML]{000000} 0.57 & {\cellcolor[HTML]{FDC088}} \color[HTML]{000000} 0.49 \\
MAHA & ViT & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 0.55 & {\cellcolor[HTML]{FDB77A}} \color[HTML]{000000} 0.53 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 0.62 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 0.08 & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 0.61 & {\cellcolor[HTML]{812804}} \color[HTML]{F1F1F1} 0.02 & {\cellcolor[HTML]{FFF3E7}} \color[HTML]{000000} 0.60 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 0.23 & {\cellcolor[HTML]{FEE5CB}} \color[HTML]{000000} 0.49 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 0.43 & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 0.60 & {\cellcolor[HTML]{FDC997}} \color[HTML]{000000} 1.19 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 0.54 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 0.05 & {\cellcolor[HTML]{FEE3C8}} \color[HTML]{000000} 0.22 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 0.81 & {\cellcolor[HTML]{FDC28B}} \color[HTML]{000000} 1.79 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 0.09 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.21 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.22 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 0.22 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 0.22 \\
\bottomrule
\end{tabular}
